RadContour: Can Frozen Multimodal LLMs Segment 3D Medical Images?

Segmenting anatomies and pathologies in 3D medical images underpins diagnosis, treatment planning, and disease monitoring. Yet dense 3D labels are among the scarcest data in medicine, and segmentation models trained on them generalize poorly beyond their training distribution. General-purpose Multimodal Large Language Models (MLLMs) are not trained to segment volumes, but they already know much of the anatomy and radiology a clinician describes in words. We present RadContour, a training-free pipeline that turns a frozen MLLM into a text-prompted 3D segmenter of CT, MRI, and PET volumes, drawing outlines on slices, much as radiologists contour a lesion. The MLLM is the only vision component. It plans the target from a free-text prompt, localizes it in 3D from coarse to fine, and traces closed outlines on a few keyframes. Deterministic geometry then assembles the outlines into a 3D mask. We evaluate RadContour zero-shot on 17 public CT, MRI, and PET benchmarks spanning 923 volumes. On nine tumor and lesion benchmarks, RadContour matches the mean Dice of the trained state of the art on identical cases (58.7 vs. 58.4) and more than doubles that of every other trained text-promptable model. On soft-tissue sarcoma, it nearly doubles the Dice of the best trained model (76.5 vs. 39.3). Across 25 backbone MLLMs, accuracy follows backbone strength with an unchanged pipeline.

==> preamble.tex <==

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}









==> setup.tex <==

\PassOptionsToPackage{dvipsnames,table}{xcolor}
\pdfsuppressptexinfo=-1

\usepackage[review]{cvpr}      %

\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{microtype}
\usepackage{nicefrac}
\usepackage{pifont}
\usepackage{comment}
\usepackage{soul}
\usepackage{cuted}            %
\usepackage{tikz}
\usetikzlibrary{spy}
\usepackage{makecell}
\usepackage{adjustbox}
\usepackage{booktabs}
\usepackage{pgf}
\usepackage{wrapfig}
\usepackage[most]{tcolorbox}
\usepackage{listings}
\input{commands.tex}
\input{preamble_tables.tex}
\renewcommand{\supp}{\textit{supplementary material}\xspace}

\usepackage{xr-hyper}   %
\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,allcolors=cvprblue]{hyperref}

\raggedbottom
\makeatletter
\setlength{\@fptop}{0pt}
\setlength{\@dblfptop}{0pt}
\makeatother

\newcommand{\ours}{RadContour\xspace}           %
\newcommand{\haiku}{Claude Haiku~5.5\xspace}    %
\newcommand{\sonnet}{Claude Sonnet~5.5\xspace}  %
\newcommand{\fable}{Claude Fable~5.2\xspace}    %
\newcommand{\opus}{Claude Opus~5.5\xspace}
\newcommand{\flash}{Gemini~3.8 Flash\xspace}
\newcommand{\oursh}{\ours{} (Haiku~5.5)\xspace}     %
\newcommand{\ourss}{\ours{} (Sonnet~5.5)\xspace}
\newcommand{\oursf}{\ours{} (Fable~5.2)\xspace}   %
\newcommand{\second}[1]{\underline{#1}}
\newcommand{\eqn}[1]{Eq.~(\ref{#1})}
\newcommand{\na}{{--}}
\newcommand{\tbd}{{\color{orange}\textbf{?}}}
\newcommand{\sd}[1]{{\scriptsize$\pm$#1}}
\newcommand{\missing}[1]{\colorbox{yellow!60}{\parbox{0.95\linewidth}{\footnotesize\textbf{MISSING:} #1}}}
\newcommand{\hlm}[1]{\sethlcolor{yellow}\hl{#1}}   %
\newcommand{\pend}{\hlm{--}\xspace}   %

\newlength{\qgw}
\newcommand{\qim}[1]{\includegraphics[width=\qgw]{imgs/#1}}
\newcommand{\qimh}[1]{\includegraphics[width=\qgw,height=\qgw,keepaspectratio]{imgs/#1}}
\newcommand{\qhd}[1]{{\scriptsize\textbf{#1}}}
\newcommand{\qrow}[2]{\rotatebox{90}{\parbox{\qgw}{\centering\scriptsize\textbf{#1}\\[-1pt]{\tiny\emph{``#2''}}}}}

\def\paperID{5526} %
\def\confName{CVPR}
\def\confYear{2027}

